A Survey on Privacy Attacks Against Digital Twin Systems in AI-Robotics

Industry 4.0 has witnessed the rise of complex robots fueled by the integration of Artificial Intelligence/Machine Learning (AI/ML) and Digital Twin (DT) technologies. While these technologies offer numerous benefits, they also introduce potential privacy and security risks. This paper surveys privacy attacks targeting robots enabled by AI and DT models. Exfiltration and data leakage of ML models are discussed in addition to the potential extraction of models derived from first-principles (e.g., physics-based). We also discuss design considerations with DT-integrated robotics touching on the impact of ML model training, responsible AI and DT safeguards, data governance and ethical considerations on the effectiveness of these attacks. We advocate for a trusted autonomy approach, emphasizing the need to combine robotics, AI, and DT technologies with robust ethical frameworks and trustworthiness principles for secure and reliable AI robotic systems.

==> document_dump.tex <==
%% Related work Dump 

\begin{comment}
Adversarial attacks have been intensively investigated in the area of cyber physical systems [XXX] with numerous attack methods and techniques developed mostly for XXX tasks. 
Researchers have noted the public safety risk of adversarial attacks, such as those utilized in self-driving vehicles, which might be misled into misclassifying a stop sign, possibly leading in a deadly consequence \cite{amodei2016concrete}.
In network security, the ramifications of adversarial attacks are also substantial \cite{vorobeychik2018adversarial}, especially in areas such as intrusion detection \cite{wang2018deep} and malware detection \cite{liu2018adversarial} where there has been rapid progress in the adoption of machine learning for such tasks. 
Even though adversarial machine learning has lately been actively investigated in network security, to the best of our knowledge, there is presently no publication that has assessed the large quantity of developing academic effort on adversarial machine learning in this field. 
Some existing survey studies we evaluated are Akhtar et al. \cite{akhtar2018threat} which reviewed adversarial attacks against deep learning in computer vision. 
Qui et al \cite{qiu2019review}  offered a generic study on adversarial attacks in artificial intelligence, with a brief discussion on cloud security, malware detection, and intrusion detection. 
Liu et al. \cite{liu2018survey} reviewed security vulnerabilities and corresponding defensive techniques of machine learning, focusing on the threats in the learning algorithms. Duddu el al. in \cite{duddu2018survey} studied various research works on adversarial machine learning in cyberwarfare, with some mention of adversarial attacks against malware classifiers. 
Zhang et al. \cite{zhang2019deep} mentioned adversarial attacks as a limitation of deep learning in mobile and wireless networking but did not explore deep learning in the context of network security applications. 
Buczak et al. \cite{buczak2015survey} in their survey on machine learning-based cybersecurity intrusion detection focused on the complexity and problems of machine learning in cybersecurity but did not cover adversarial attacks in their research. 
Biggio and Roli \cite{biggio2018wild} gave a historical chronology of adversarial machine learning in the area of computer vision and cybersecurity, their work did not give a full evaluation in the context of network security. 
Gardiner et al. \cite{gardiner2016security} centered their assessment on the security of machine learning in malware detection on analyzing the Call and Control (C \& C) detection methodologies. 
They also highlighted the flaws and described the limitations of secure machine learning algorithms in malware detection systems. 
Domain-specific surveys on adversarial machine learning have also been published, notably Hao et al. \cite{xu2020adversarial} in which numerous adversarial attacks and countermeasures in images, graphs, and texts were studied. 
In the field of natural language processing, zhang et.al \cite{zhang2020adversarial} evaluated many articles in which deep adversarial attacks and defenses were developed. 
Sun et al. \cite{sun2018survey} presented a survey og adversarial machine learning in graph data. Akhtar et al. 
\cite{akhtar2018threat} computer vision, Duddu et al. \cite{duddu2018survey} cyber warfare.


Research Gap With rising interest in the use of machine learning for network security applications, the relevance of adversarial attacks against such machine learning-based applications has grown more widespread. 
With the ongoing expansion in the volume of work in this field, there have been new initiatives to examine these articles as survey work. 
In the field of network security, we discovered survey papers that aim to examine adversarial machine learning in the context of network security. 
None of these previous survey papers have, however, explored the vast amount of ongoing research on the topic of adversarial machine learning in network security in a manner that categorizes them based on security applications, problem and feature space dimensional classification, and an adversarial risk grid map. 
Our study, more importantly, aims to differentiate between adversarial attacks in general and adversarial machine learning in context. 
We emphasize that an adversary may strive to compromise network security applications in many ways, and this may not be connected to adversarial machine learning. 
For example, in \cite{corona2013adversarial} where adversarial attacks on intrusion detection systems were studied, in our context, adversarial machine learning specifically addresses the optimization issue in which a machine learning-based network security solution is being attacked. Many network security solutions are strictly rule-based or hard programming dependant and do not incorporate machine learning approaches. 
Our study work does not relate to such adversarial attacks since they do not describe the genuine setting of adversarial machine learning in principle.


\end{comment}


\begin{comment}
    %%%% Adversarial attack classification


\subash{Taxnomony of attacks --resource --https://tinyurl.com/4nnv9m2u -refer this}

\hl{Milan 1 page}\\
Adversarial attacks have become a severe threat to the present AI system. 
In the age of the Internet of Everything, the network has become the ideal target for cyber attackers. 
Vulnerabilities in artificial intelligence are routinely exploited by attackers to launch cyberattacks.
Based on gradient descent and L-norm optimization techniques, Liu et al. \cite{liu2019atmpa} originally published the method to exploit a malware-based visual detector for adversarial example attacks.
Zhou et al. \cite{zhou2020dast} were the first to suggest an alternate methodology for training adversarial attacks without real data.


Spect et al. (2018) FGSM attack was used to generate adversarial samples, that were classified by the ML model as normal sensory data (White box evasion attack)

Erba et al. (2019) Enumerate all possible operations for every sensor and use the coordinate descent algorithm for generating adversarial samples (White box and black box evasion attacks)

\begin{comment}
\subsection{Adversarial Attacks}


\subsubsection{Concepts}
In this subsection, some common terms used in the literature related to adversarial attacks are presented.

\subsubsection{Adversarial Example}
An adversarial example is an artificially constructed example that makes machine learning models misjudge by adding subtle perturbations to the original example but at the same time does not make human eyes misjudge [XXX].

\subsubsection{White-Box Attack}
White-box attacks assume that the target model can fully obtain the structure of the model, including the composition of the model and the parameters of the partition layer, and can fully control the input of the model [XXX].

\subsubsection{Black-Box Attack}
Black-box attacks have no idea of the internal structure of the model and can only control the input and carry out the next attack by comparing the feedback of the input and output [XXX].

\subsubsection{Real-World Attack/Physical Attack}
Real-world attacks/physical attacks do not understand the structure of the model and even have weak control over the input [XXX].

\subsubsection{Targeted Attack}
Targeted attacks will set the target before the attack, causing it to incorrectly predict the specific label of the adversarial images, which means that the effects after the attacks are determined [XXX].

\subsubsection{Untargeted Attack}
Untargeted attacks do not need to set the target before the attack, as long as the result of identification is wrong after the attack [XXX].

\subsubsection{Evade Attack}
Evade attacks refer to adding disturbance to test samples and modifying the input during the test phase, to avoid or deceive the detection of the model and make the AI model unable to be correctly identified [XXX].

\subsubsection{Poisoning Attack}
By adding carefully constructed malicious examples in the model training phase, poisoning attacks make the trained model have a backdoor or vulnerability, which can be used by attackers to carry out attacks [XXX].

\subsubsection{Backdoor Attack}
A backdoor attack means that the attacker can enter the system without identity authentication, which means that the attacker can bypass the security control to gain access to the system and even further damage the computer or network. The neural network backdoor attack referred to in this paper refers to the attacker generating a model with a backdoor by implanting specific neurons in the neural network model, so that the judgment of the model on normal inputs is consistent with the original model, but the judgment on special inputs will be controlled by the attacker [21]. A backdoor attack is a type of poisoning attack [XXX].


\subsubsection{Detection Model}
The detection model means to detect whether the examples to be judged are adversarial examples by detecting components. Various detection models may judge whether the input is an adversarial example according to different criteria [XXX].


Adversaries can alter data in the training and testing phase, according to \cite{qiu2019review} there are 5 different ways for modification of data as illustrated in Table \ref{tab: adverserial_attack}. First we will describe what training and testing stage are and subsequently showcase examples state-of-the-art research of each factor listed in Table XXX.

\subsubsection{Training Stage}:
Adversarial attacks in the training phase mean during the training phase of the target model, adversaries attack by altering the training dataset and modifying input features. This kind of attack will impact the input data and significantly influence the results of the target model.  

\subsubsection{Testing Stage}:
Adversarial attacks in the testing stage can be split into two attack types such as white box and black boxes. Adversaries have access to the parameter, algorithms, and structure of the target model in white-box scenarios whereas, in black box scenario the adversaries don’t have explicit information about the target model however, they are capable of training a local substitute model by querying the target model. This is executed either by utilizing the transferability of adversarial samples or using a model inversion method. 

In adversarial attacks, attackers attempt to perturb a data point $x$ to an adversarial data point $x'$ so that $x'$ is misclassified by an model with high confidence, although $x'$ is visually indistinguishable from its original data point $x$ by humans. \hl{maybe we can give some example}. 
Adversarial attacks can be conducted in different application domains, such as audio [XXX], text [XXX], network signals [XXX], and images [XXX]. 
They can be further classified based upon the knowledge level that adversaries maintain about a target model. 
The attack model can be specified as either \emph{black-box}, \emph{white-box}, or \emph{gray-box}. \emph{Black-box} attacks refer to the case when an attacker has no access to the trained model. 
Instead, the attacker only knows the model outputs (logit, confident score, or label). \emph{Black-box} attacks are commonly observed in online learning techniques used in anomaly detection systems that effectively retrain the detector when new data is available. 
In a \emph{gray-box} attack, attackers may have some incomplete knowledge about the overall structure of a target model. 
Last, in a white-box threat model, attackers have complete knowledge about a target model, which therefore facilitates the task of generating adversarial examples and crafting poisoned input data. 
Even though there are more white-box attacks among the three types of attacks, \emph{black-box} attacks are more practical attacks on ML systems because essential model information is often confidential and protected from a normal user interacting with a system. 
Furthermore, due to the phenomenon of attack transferability, \emph{white-box} attacks can be utilized to attack black-box models (transfer attacks). 

In data poisoning attacks, adversaries try to manipulate training data in an attempt
\begin{enumerate}
    \item to decrease the overall performance (i.e., accuracy) of an model,
    \item to induce misclassification in a specific test sample or a subset of the test sample, or
    \item to increase training time.
\end{enumerate}

If an attacker has a specified target label for which a specific test sample is misclassified, the attack is called a targeted data poisoning attack; otherwise, it is called an untargeted data poisoning attack. 
Adversaries are assumed to either be able to contribute to the training data or have control over the training data. 
For instance, crowdsourcing is regarded as a vital data source for various smart cities, such as intelligent transportation systems, and traffic monitoring [XXX]. 
Hence, such systems are vulnerable to data poisoning threats [XXX] as data poisoning attacks are often difficult to detect [XXX].

\subsection{Training Phase Attacks}
\subsubsection{Model Poisioning}
The adversary can poison the training dataset. To achieve this, the adversary derives and injects a point to decrease the classification accuracy [XXX]. This attack has the ability to completely distort the classification function during its training thus allowing the attacker to define the classification of the system in any way she wishes. The magnitude of the classification error depends on the data the attacker has chosen to poison the training. With regards to the aforesaid example, the adversary may be able to create dataset of anomalous network-layer protocol behaviour and train an anomaly-based intrusion detection system with a labelled attack dataset as the groundtruth. As a result, the detector will not be able to recognize cyber attacks against this network-layer protocol threatening the security of the underlying system. This attack could be tailored to also have a significant impact to the quality of a signature-based intrusion detection system, which is responsible, for example, for detecting malware infecting a system or an infrastructure.

For example, a particularly insidious attack in this category is the backdoor or Trojan attack, where the adversary carefully poisons the model by inserting a backdoor key to ensure it will perform well on standard training data and validation samples, but misbehaves only when a backdoor key is present [XXX]. Thus an attacker can selectively make a model misbehave by introducing backdoor keys once the model is deployed. For instance, consider the case of assistive driving in autonomous vehicles: a backdoor could cause the model to misclassify a stop sign as speed limit whenever a specific mark has been placed on the stop sign. However, the model would perform as expected on stop signs without this mark, making the backdoor difficult to detect since users do not know the backdoor key a priori.

\subsection{Deployment Phase Attacks}
\subsubsection{Evasion}
The adversary can undertake an evasion attack against classification during the testing phase thus producing a wrong system perception. In this case, the goal of the adversary is to achieve misclassification of some data towards, for example, remaining stealthy or mimicking some desirable behaviour. With regards to network anomaly-based detection, an intrusion detection system (IDS) can be evaded by encoding the attack payload in such a way that the destination of the data is able to decode it but the IDS is not leading to a possible misclassification. Thus, the attacker can compromise the targeted system being spotted out by the IDS. An additional goal of the attacker could be to cause concept drift to the system leading to continuous system re-training, thus, significantly degrading its performance [XXX].
\end{comment}

    
\end{comment}

\begin{commnet}

Numerous research \cite{das2018taxonomy} \cite{hansman2005taxonomy} have endeavored to separate the different domains of network security into multiple fragmented domains. 
A popular technique, for example, make attempts at distinguishing malware and spam detection from intrusion detection \cite{rosenberg2020adversarial}. 
%We find that this attempt at fine-grained classification results in duplication since the job of malware or phishing detection in a network might be regarded as an intrusion detection task. 
%As a result, we define cyberattacks against a network in this study as an effort by an adversary to infiltrate the network with a malicious payload. 
We identify three major categories of malicious payload in a network: malicious files (malware), malicious text (spam), and malicious URL links (phishing). 
We point out that most cyberattacks by attackers may combine all three payloads. 
For instance, a malicious file attachment or a link to a malicious website could be contained in a spam email.
In our study on adversarial attacks in the area of network security, the payload technique becomes even more significant.
%Our study has led us to the conclusion that, in contrast to other domains like computer vision, the network security domain plays a critical role in giving an accurate categorization of adversarial attacks.
We present a classification method for adversarial attacks in network security in this section that is based on network security tasks.
Our classification method investigates the data object being manipulated by the adversary.
The data object correlates to the feature span of the adversarial attack, as shown in \ref{figs:Adv_Attack_Classi}.
%We evaluate adversarial attacks based on the actual payload that is being targeted in context for the purposes of this research.
The payload refers to the part of the transferred data that truly contains the message that is meant to be sent from the sender to the receiver.
For instance, the payload represents the portion of the transmitted data, i.e., the message text, files, and Website links when an email when is sent.
%Within the framework of our research, identifiers, and metadata that help deliver the payload are not regarded as a component of the payload.
%As a result, the protocol delay is not regarded as actual data.
This is the basis for our method of classifying adversarial attacks in network security, as shown in \ref{figs:Adv_Attack_Classi}. 
This is referred to as feature scope-based categorization, and it relates to which features the attacker manipulates or perturbs in order to generate an adversarial sample. 
Adversarial assaults aim to disrupt the payload features, such as a binary file, a URL, or an email message, in malware detection, phishing detection, and spam detection applications.
These are classified as adversarial attacks on endpoint security systems.
On the other hand, adversarial attacks are also made against applications that identify network anomalies, and they aim to disrupt protocol features like network information or protocol headers.
These attacks are categorized as adversarial attacks on network defenses.

Malware detection, phishing detection, spam detection, and network anomaly detection are the four general groups of network security areas that employ machine learning techniques. 
Fig. 1 demonstrates this classification, where endpoint-based protection is referred to as the first three types of network security tasks. 
This group of endpoint-based security includes machine learning apps that are usually started with payload features. 
Machine learning applications in this area are usually started with protocol features and focus on network security, which is mainly comprised of network anomaly detection. 
%Passive assaults like spying are outside the purview of this research because it only examines active attacks against a network. 
%Specific data items are used by adversarial assaults to create adversarial examples.


\begin{figure}[h]
\centering
\includegraphics[scale = 0.066]{figs/Adv_Attack_Classi.png}
\caption{Adversarial attack classiﬁcation}
\label{figs:Adv_Attack_Classi}
\end{figure}

\begin{comment}
In this section, we describe the main methods for generating adversarial examples in the image, text, and malware domains. And the work of some researchers is reviewed. Adversarial machine learning is a widely used technology in the field of image, and the research has been quite comprehensive. 
The malicious code domain and the text domain are similar and can be borrowed from each other. 
Figure 1 is the classification of image-based adversarial attacks. 
According to the attacker’s knowledge, the attack can be divided into a black-box attack, a white-box attack, and a physical attack. 
Figure 2 is the classification of text-based adversarial attacks. 
According to the access permissions of the model, the attack can be divided into black-box attacks and white-box attacks. 
And according to the effect after the attack, it can be divided into targeted attack and nontargeted attack. 
Moreover, according to the text granularity, it can be divided into character level, word level, and sentence level. 
Besides, the attack strategy can be divided into image-to-text, importance-based, optimization-based, and neural network-based. 
Figure 3 is the classification of malware-based adversarial attacks. 
According to the object, it can be divided into attacks on training data and attacks on a neural network model.

\begin{figure}
\centering
\includegraphics[scale = 0.07]{figs/image-based.png}
\caption{Classification of image-based adversarial attack.}
\label{figs:dT_dfd_architecture}
\end{figure}

\begin{figure}
\centering
\includegraphics[scale = 0.07]{figs/text-based.png}
\caption{Classification of text-based adversarial attack.}
\label{figs:dT_dfd_architecture}
\end{figure}

\begin{figure}
\centering
\includegraphics[scale = 0.07]{figs/malware-based.png}
\caption{Classification of malware-based adversarial attack.}
\label{figs:dT_dfd_architecture}
\end{figure}



\subsection{Hazards}
The main harm of adversarial attack includes the following:
\begin{enumerate}
    \item Model losing or stealing: network information data has become the most precious intangible asset in the current Internet of Everything era. In the current era of the Internet of Everything, network information data has become the most precious intangible asset. Plenty of adversarial attacks are designed to steal secret data, such as stealing privacy data from computers or servers and after that deceiving or blackmailing victims. More malicious attacks are aimed at enterprises to steal valuable trade secrets from enterprises and obtain economic benefits, even worse, targeting a country and stealing national security-related intelligence information from government departments for strategic purposes
    \item Model failure: the adversarial attack causes the failure of the deep learning model and makes it unable to work properly utilizing physical attack against the vulnerability of the model. For instance, in the field of autonomous driving, the superposition of image data with subtle perturbations makes it difficult for humans to recognize by senses, which leads to the wrong classification decision made by the machine learning model and causes traffic accidents
    \item Data poisoning: a typical scenario is the recommendation system. When hackers add abnormal data to the training samples of deep learning, the most direct impact is that the classification error of the deep learning model, i.e., the recommendation system, generates an error
    \item Other hidden hazards: apart from the obvious harms mentioned above, adversarial attacks can also cause some hidden hazards. For instance, many malware generate adversarial examples through some algorithms, and the malicious behavior does not change, but the detection of antivirus systems fails, which eventually leads to malicious attacks on computers and networks as well as losses of profits.
\end{enumerate}
\end{comment}

\end{commnet}

\begin{comment}
    %%% adversarial deep learning
Adversarial attacks have been researched for over a decade now \cite{XXX}. 

The adversary achieves this by modifying the input data that is fed to the machine learning model either during the training phase (poisoning attack) \cite{XXX} or during the inference phase (evasion attack) \cite{XXX}. 
The reason behind adversarial examples has been linked to the fact that most machine learning models remain overly attached to the superficial statistics of the input data \cite{XXX} \cite{XXX}. 
This attachment to the input data makes the machine learning highly sensitive to distribution shifts, resulting in a disparity between semantic changes and a decision change \cite{XXX}. 
The attack surface, threat model, adversarial framework, and adversarial risk are all components of the security model for using machine learning in network security. 
An alternative adversarial model was proposed in \cite{XXX} which modeled the adversary using a three-fold approach based on knowledge, goals, and capability.
The attack surface identifies the various attack vectors along a typical machine-learning data processing pipeline in network security-related applications. 
The threat model provides a system abstraction for profiling the adversary’s capabilities and the potential threats that are associated. 
The adversarial framework details our approach for classifying the various attacks and defenses within each network security domain, and lastly, the adversarial risk provides an evaluation of the likelihood and severity of adversarial attacks within a network security system. 
A major component of an adversarial attack is the adversarial sample. 
An adversarial sample consists of an input to a machine-learning model that has been perturbed. For a particular dataset with features x and label y, a corresponding adversarial sample is a specific data point $x’$  which causes a classifier c to predict a different label on $x’$  other than $y$ , but $x’$ is almost indistinguishable from x. 
The adversarial samples are created using one of many optimization methods known as adversarial attack methods. 
Crafting adversarial samples involves solving an optimization problem to determine the minimum perturbation that maximizes the loss for the neural network. 
Given an input $x$  and a classifier $f$, the adversary's optimization goal is to compute a perturbation with a small norm, measured against some distance metric, that modifies the classifier's output in such a way that:

\begin{equation}
f (x + \delta) \neq f(x)
\end{equation}

where $\delta$ is the perturbation. 

Adversarial machine learning in network security is typically an arms race between two agents. 
The first agent is an adversary whose objective is to intrude on a network with a malicious payload. 
The other agent is one whose role is to protect the network from the consequences of the malicious payload.  
We start with a view of the different types of data that traverses a network at any given time.

\begin{figure}
\centering
\includegraphics[scale = 0.07]{figs/AdvAttack_Taxonomy.png}
\caption{Adversarial attack classification}
\label{figs:AdvAttack_Taxonomy}
\end{figure}

\begin{figure}
\centering
\includegraphics[scale = 0.25]{figs/AdvMachineLearning.png}
\caption{Adversarial Machine Learning}
\label{figs:AdvMachineLearning}
\end{figure}
    
\end{comment}


\begin{comment}
    %%% adversarial threat model

We examine the threat model in Figure \ref{figs:AdvAttack_Taxonomy} to consider the goals and capabilities of any adversary for a machine learning system. We base our threat framework on the
original model in \cite{XXX} \cite{XXX} and adapt it within the context of adversarial attacks in the network security domain. Within this context, adversarial attack threats in network security may be considered based on the attacker’s knowledge, attack space, attacker’s strategy, attacker’s goal, and attack target.  

\begin{enumerate}
    \item Knowledge: The adversarial threat model's knowledge component explains how much the adversary understands the computer system as a whole. This could be a "white box," "gray box," or "black box" attack.

It is presumed in white-box attacks that the adversary is fully aware of the training data, the learning method, the learned model, as well as the parameters that were applied during the model's training. An adversary carrying the precise knowledge possessed by the owner or creator of the machine learning system that is being attacked is represented by a white-box assault. This is typically not possible in the majority of adversarial attack situations encountered in the real-world.      
A Gray-box attack takes a more practical strategy, recognizing that the adversary may have access to different degrees of knowledge, \cite{XXX}. An adversary, for example, may have only incomplete knowledge of the model queries or restricted access to the training data. In a gray-box attack, the adversary lacks the precise knowledge that the model's author holds, but he or she has enough information to attack the machine-learning system and cause it to fail.   
A black-box attack assumes that the adversary is totally unaware of the machine-learning system. In this type of attack, the adversary has no knowledge about either the learning algorithm or the learned model. It may be argued that a truly black-box attack is impossible. This is because it is assumed that the adversary must at least have some specific information, for example, the location of the model, before it can attack it. The severity of black-box attacks poses a greater threat in practice. The model for real-world systems may be more restrictive than a theoretical black-box model where the adversary can understand the full output of the neural network based on inputs that have been chosen arbitrarily. In \cite{XXX}, an analysis of three threat models was proposed. These models, defined as, the query-limited setting, the partial information setting, and the label-only setting, provide a more accurate characterization of real-world classifiers. As such, a representation of black-box adversarial attacks was proposed, such that, it would be possible to fool classifiers under these more restrictive threat models, whereas, it might have been impractical or ineffective.

An adversary is considered to be completely ignorant of the machine learning system in a black-box assault. The adversary in this kind of attack is ignorant of both the learning method and the learned model. One could contend that a true black-box attack is impractical. This is because it is believed that in order to target a model, the adversary must at the very least know where the model is. Black-box attack's seriousness makes them a bigger danger in real life. The adversary can fully comprehend the output of the neural network based on inputs that have been selected randomly in a theoretical black-box model, but the model for real-world systems may be more constrained. A study of three danger models has been put forth in citation \cite{XXX}. These models—described as the query-limited setting, the partial information setting, and the query-limited setting—offer a more true representation of classifications used in the real world. As a result, a depiction of black-box adversarial attacks was suggested, making it feasible to trick classifiers under these more limited threat models, whereas it might have been difficult or ineffectual to do so under less constrained threat models.


    
    \item Space:  In the field of adversarial machine learning, the input space can be defined as a dimensional representation of all the possible configurations of the objects in the determination context. We categorize this as Feature Space and Problem Space.
    \begin{itemize}
        \item Feature space modeling of an adversarial sample is a method in which an optimization algorithm is used to find the ideal value out of a finite number of arbitrary changes made to the features. In a feature space adversarial attack, the attacker’s objective is to remain benign without generating a new instance. Conversely, a feature space is defined as the n-dimensional space in which all variables in the input dataset are represented.  A feature space attack modifies the features in the instance directly. Using an example of malware adversarial attacks, a feature space adversarial malware attack will only modify the feature vectors but no new malware is created.
        \item The problem space refers to an input space in which the objects e.g. image, file, etc. resides. A problem space adversarial malware attack will modify the actual instance from the source to produce a new instance of the malware. Typically, a problem space adversarial attack tends to generate new objects in domains such as malware detection whereby there is no clear inverse mapping to the feature space \cite{XXX}. A typical difference between a problem space adversarial attack, and a feature space adversarial attack is that a feature space attack does not generate a new sample but only creates a new feature vector. A problem space adversarial attack modifies the actual instance itself to create an entirely new object.
    \end{itemize}
    \item  Strategy: Attacker’s strategy implies the phases of operation in which the adversary launches the attack. Three main strategies which an adversary may use in adversarial attacks are Evasion, Poisoning, and Oracle.
    \begin{itemize}
        \item Evasion attacks, also known as exploratory attacks or attacks during the decision-making, testing, or inference phase. The attacker aims to confuse the decision of the machine learning model after it has been learned as shown in Figure 6. Evasion attacks typically involve an arithmetic computation of an optimization problem. The goal of the optimization problem is to compute a small perturbation sigma, which results in an increase in the loss function. The change in loss function would The difference must then be significant enough for the machine learning model to make an incorrect prediction. Evasion attacks are classified as gradient-based attacks or gradient-free attacks. Gradient-based attacks are further classified based on the frequency with which the adversarial samples are updated or optimized. These are iterative or one-shot attacks. Iterative attacks provide tighter control of the perturbation in order to generate more convincing adversarial samples \cite{XXX}. This, however, results in higher computational costs. Alternatives to iterative attacks are one-shot attacks that adopt a single-step approach without iterations. One-shot or one-time attacks are attacks in which the adversarial samples are optimized just once. Iterative attacks, however, involve updating the adversarial samples multiple times. By updating the adversarial samples multiple times, the samples are better optimized and perform better compared to one-shot attacks. However, iterative attacks cost more computational time to generate. Adversarial attacks against certain machine learning techniques that are computationally intensive, such as reinforcement learning usually demand one-shot attacks as the only feasible approach [69]. Gradient-free attacks \cite{XXX}, unlike gradient-based attacks do not require knowledge of the model. Gradient-free attacks can generate potent attacks against a machine-learning model with knowledge of only the confidence values of the model.

        \item Poisoning attacks, also known as causative attacks, involve adversarial corruption of the training data or model logic during the training phase to induce a wrong prediction from the machine learning mode, as shown in Figure XXX. Poisoning attacks may be carried out by data injection, data manipulation, or logic corruption \cite{XXX}. Data injection occurs when the adversary inserts adversarial inputs to alter the data distribution while preserving the original input features and data labels. Data manipulation refers to a situation in which either the input features or data labels of the original training data are modified by the adversary. Logic corruption is an attempt by the adversary to model structure.

        \item Oracle attacks occur when an adversary leverages access to the Application Programming Interface of a model, to create a substitute model with malicious intent. The substitute model typically preserves a significant part of the functionality of the original model \cite{XXX}. As a result, the substitute model can then be used for other types of attacks such as evasion attacks \cite{XXX}. Oracle attacks can be further subdivided into Extraction, Inversion, and Inference attacks. The objective of an extraction attack is to deduce model architectural details such as parameters and weights from an observation of the model’s output predictions and class probabilities \cite{XXX}. Inversion attacks occur when the adversary attempts to reconstruct the training data. An inference attack allows the adversary to identify specific data points with the distribution of the training dataset \cite{XXX}. 
        \end{itemize}
    \item   Goal: Traditionally in the field of computer vision, adversarial attacks are regarded in terms of targeted or reliability attacks \cite{XXX}. In targeted attacks, the attacker has a specific goal with regard to the model decision. Most commonly, the attacker would aim to induce a definite prediction from the machine learning model. On the other hand, a reliability attack occurs when the attacker only seeks to maximize the prediction error of the machine learning model without necessarily inducing a specific outcome. Yevgeny et al. \cite{XXX} have noted that the distinction between reliability and targeted attacks becomes blurred in attacks on binary classification tasks such as malware binary classification. As such, these conventional paradigms of attacker goal classification are not optimal for consideration in network security. We choose to adopt the CIA triad in this context and find that it is more suitable for adversarial classification of the adversary goals in the network security domain.
    \begin{itemize}
        \item Confidentiality attack refers to the goal of the attacker to intercept communication between two parties A and B, to gain access to private information being exchanged. This happens within the context of adversarial machine learning, whereby machine learning techniques are being used to carry out network security tasks.
        \item Integrity attack seeks to cause a misclassification, different from the actual output class that the machine learning model was trained to predict. An integrity attack could result in a targeted misclassification or a reliability attack. A targeted misclassification attempts to cause the machine learning model to make a specific incorrect prediction. A reliability attack either reduces confidence or causes misclassification of any array class other than the correct one.
        \item Availability Attack results in a denial of service situation for the machine learning model. as a result, the machine earning model becomes either totally unavailable to the user, or the quality is significantly degraded to the extent that the machine learning system becomes unusable to the end users.
    \end{itemize}
    \item  Target: We consider the model which is being targeted in our threat model based on the various machine learning techniques which we discussed in section III. In our surveyed work, adversarial attacks are targeted against a specific machine-learning technique. Several successful attempts have been made toward the transferability of adversarial attacks \cite{XXX} \cite{XXX}. However, attacks that have been targeted toward a specific machine learning technique for example unsupervised learning, have not been successfully transferred toward another technique for example supervised learning.
\end{enumerate}



%%%%%%%% Adversarial Attack Taxonomy ##########

\begin{figure*}[h]
\centering
\includegraphics[scale = 0.14]{figs/AdvAttack_Taxonomy.png}
\caption{Adversarial attack architecture against a trained digital twin.}
\label{figs:architecture}
\vspace{-4mm}
\end{figure*}



%%%%%%%% Subash Figure ##########
\begin{figure*}[h]
\centering
\includegraphics[scale = 0.67]{figs/Adversarial_DT.pdf}
\caption{Adversarial attack architecture against a trained digital twin.}
\label{figs:architecture}
\vspace{-4mm}
\end{figure*}



%%%%%%%% Ivan Figure  ##########
\begin{figure*}[h]
\centering
\includegraphics[scale = 0.5]{figs/Temp_FlowDiagram.pdf}
\caption{Adversarial training framework.}
\label{figs:architecture2}
\vspace{-4mm}
\end{figure*}
    
\end{comment}

==> table_dt_intro.tex <==
\begin{table}[ht]
{\renewcommand{\arraystretch}{1.30}%
\caption{Digital Twin modeling for Robotic Systems.}
\vspace{-2mm}
%\begin{tabularx}{\textwidth}{X|X|X|X|X|X|X}
%\begin{tabularx}{\textwidth}{X|X|X|X|X|X}
\begin{tabular}{p{1.2cm}|p{2.3cm}|p{4.0cm}}
%\begin{tabular}{p{3.4cm}|l|l}
\hline
\rowcolor{cyan!20!}
\textbf{Name} & \textbf{Representation}  & \textbf{DT Modeling} \\ \hline

%%%% Sense %%%%%%
\multirow{3}{*}{Component} & A fundamental constituent of a larger system. & A DT can model a specific component of a robotic system such as a sensor or an actuator.\\ \hline
%%%% end Sense %%%%%%                                    

%%%% Plan %%%%%%    

System of Components & A complex system is comprised of many components. & A DT can model a robotic system by having a virtual representation for each of its components. \\ \hline

%%%% end Plan %%%%%%                           

%%%% Act %%%%%%
System of Sytems (SoS) & Complex systems interacting with each other. & A DT can model robotic systems interacting with other complex systems.\\ \hline

%%%% end Act %%%%%%
                                    
\end{tabular}}


\label{table:dt_intro}
\vspace{-2mm}

\end{table}
